Dynamic Modeling and Control of a Two-Reactor Metal Hydride Energy Storage System

Metal hydrides have been studied for use in energy storage, hydrogen storage, and air-conditioning (A/C) systems. A common architecture for A/C and energy storage systems is two metal hydride reactors connected to each other so that hydrogen can flow between them, allowing for cyclic use of the hydrogen. This paper presents a nonlinear dynamic model and multivariate control strategy of such a system. Each reactor is modelled as a shell-and-tube heat exchanger connected to a circulating fluid, and a compressor drives hydrogen flow between the reactors. We further develop a linear state-space version of this model integrated with a model predictive controller to determine the fluid mass flow rates and compressor pressure difference required to achieve desired heat transfer rates between the metal hydride and the fluid. A series of case studies demonstrates that this controller can track desired heat transfer rates in each reactor, even in the presence of time-varying circulating fluid inlet temperatures, thereby enabling the use of a two-reactor system for energy storage or integration with a heat pump.

==> OLD_02b_Model_Validation.tex <==
\subsection{Simulation Results}

\par To determine the suitability of the linear state-space model for use in controller design, the dynamics predicted by the linear model are compared to those predicted by the nonlinear model for a given set of input conditions.  To compare the models, the linear and nonlinear governing equations are implemented in Matlab and solved using a variable-step solver for stiff problems that uses a fifth-order numerical differentiation formula. We consider two cases.  In Case 1, the initial conditions are set so that hydrogen moves from reactor A to reactor B, and each model is simulated for 10 minutes (600 seconds), as shown in Figures ~\ref{fig:Case1_lin_perf} and ~\ref{fig:Case1_lin_perf_heat}.  In Case 2, the initial conditions are defined such that hydrogen flows from reactor B to reactor A, as shown in Figures ~\ref{fig:Case2_lin_perf} and ~\ref{fig:Case2_lin_perf_heat}. In both simulations, the compressor pressure difference is increased by 50 kPa after $t=5$ minutes. The initial values of the state variables ($x_{0}$) and the input and disturbance variables ($u_{0}$) for these two simulations are listed in \ref{tab:in_var}, and each simulation is initialized at the linearization point $(x_0,u_0)$.

\begin{table}[!htb]
\caption{Initial values for the state and input variables} 
\begin{center}
%\small
  \begin{tabular}{l c c c}
  \noalign{\vskip -1.5mm}
  \hline
  \noalign{\vskip 1mm}
  $\textbf{\text{ Variable}}$ & $\textbf{\text{Case 1}}$ & $\textbf{\text{Case 2}}$ & $\textbf{\text{Units}}$\\
  \noalign{\vskip 1mm}
  \hline
  \noalign{\vskip 1mm}
    $T_{A}$  & 6.89 & 6.89 & \degree C \\
    $T_{B}$ & 37.9 & 32.9 & \degree C \\
    $P_{A}$  & 480 & 310 & kPa \\ 
    $P_{B}$ & 280 & 310 & kPa \\
    $w_{A}$ & 0.006 & 0.007 & kg H / kg M \\
    $w_{B}$ & 0.006 & 0.007 & kg H / kg M \\
    $\dot{m}_{A}$  & 0.2 & 0.2 & kg/s \\
    $\dot{m}_{B}$ & 0.2 & 0.2 & kg/s \\
    $\Delta P_{comp}$  & 210 & 40 & kPa \\ 
    $T_{wg,in,A}$ & 1.89 & 11.9 & \degree C\\
    $T_{wg,in,B}$ & 42.9 & 30.9 & \degree C \\
  \noalign{\vskip 1mm}
  \hline
  \end{tabular}
\end{center}
\label{tab:in_var}
\end{table}

\begin{figure}[!htb]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_tempA.jpg}
         \caption{Temperature in Reactor A}
         \label{fig:tempA_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_tempB.jpg}
         \caption{Temperature in Reactor B}
         \label{fig:tempB_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_pressA.jpg}
         \caption{Pressure in Reactor A}
         \label{fig:pressA_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_pressB.jpg}
         \caption{Pressure in Reactor B}
         \label{fig:pressB_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_weightA.jpg}
         \caption{Weight Fraction in Reactor A}
         \label{fig:weightA_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_weightB.jpg}
         \caption{Weight Fraction in Reactor B}
         \label{fig:weightB_case1}
     \end{subfigure}
        \caption{State variables for Reactors A and B comparing the linear model (solid lines) to the nonlinear model (dashed lines) for Case 1 (hydrogen flowing from reactor A to reactor B).}
        \label{fig:Case1_lin_perf}
\end{figure}

\begin{figure}[!htb]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_heatA.jpg}
         \caption{Reactor A}
         \label{fig:heatA_case1}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case1_heatB.jpg}
         \caption{Reactor B}
         \label{fig:heatB_case1}
     \end{subfigure}
     \caption{Heat transfer rates out of Reactors A and B comparing the linear model (solid lines) to the nonlinear model (dashed lines) for Case 1 (hydrogen flowing from reactor A to reactor B).}
        \label{fig:Case1_lin_perf_heat}
\end{figure}

\begin{figure}[!htb]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_tempA.jpg}
         \caption{Temperature in Reactor A}
         \label{fig:tempA_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_tempB.jpg}
         \caption{Temperature in Reactor B}
         \label{fig:tempB_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_pressA.jpg}
         \caption{Pressure in Reactor A}
         \label{fig:pressA_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_pressB.jpg}
         \caption{Pressure in Reactor B}
         \label{fig:pressB_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_weightA.jpg}
         \caption{Weight Fraction in Reactor A}
         \label{fig:weightA_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_weightB.jpg}
         \caption{Weight Fraction in Reactor B}
         \label{fig:weightB_case2}
     \end{subfigure}
        \caption{State variables for Reactors A and B comparing the linear model (solid lines) to the nonlinear model (dashed lines) for Case 2 (hydrogen flowing from reactor B to reactor A).}
        \label{fig:Case2_lin_perf}
\end{figure}

\begin{figure}[!htb]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_heatA.jpg}
         \caption{Reactor A}
         \label{fig:heatA_case2}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Case2_heatB.jpg}
         \caption{Reactor B}
         \label{fig:heatB_case2}
     \end{subfigure}
     \caption{Heat transfer rates out of Reactors A and B comparing the linear model (solid lines) to the nonlinear model (dashed lines) for Case 1 (hydrogen flowing from reactor A to reactor B).}
        \label{fig:Case2_lin_perf_heat}
\end{figure}

\par For case 1, the linear model tracks the nonlinear model very closely, but not for case 2. In case 1, the linear model generally matches the trend for each variable, but differs in the magnitude. In both cases, the increase in the pressure difference produced by the compressor after 5 minutes does not significantly affect the accuracy of the model. In both cases, the accuracy is similar before and after the step change in compressor pressure.

\par Considering the state variables in Figure \ref{fig:Case1_lin_perf}, the fastest response in the system is the response of the reactor pressure to the change in the pressure difference between the reactors (which includes the pressure difference created by the compressor). In this initial study, this occurs at $t=5$ minutes when the compressor pressure difference is increased. It results in an almost immediate step change in the pressure of reactor A approximately equal to the change in the compressor pressure difference, as seen in Figure \ref{fig:pressA_case1}. The change in pressure occurs primarily in reactor A because at this operating condition, the reaction rate in reactor B is more sensitive to changes in pressure than the reaction rate in reactor A. When the compressor pressure difference increases, the mass flow rate between the reactors increases, becoming much larger than the absorption rate in reactor A or the desorption rate in reactor B. Since hydrogen is flowing from reactor B to reactor A, this results in the pressure in reactor A increasing and the pressure in reactor B decreasing. However, since magnitude of the the reaction rate increases much faster in reactor B, the pressure there stops decreasing (due to increased desorption balancing out increased flow into the reactor) sooner than the pressure in reactor A stops increasing, and thus the pressure in reactor A increases much more than the pressure in reactor B decreases, as can be seen by comparing Figure \ref{fig:tempA_case1} to Figure \ref{fig:tempB_case1}. This process occurs in a few seconds- (insert quantifiable metric here)- and therefore appears as a step change when plotted against a 10-minute time span in Figure \ref{fig:Case1_lin_perf}. The linear state-space model successfully captures this response: as seen in Figures \ref{fig:tempA_case1} and \ref{fig:tempB_case1}, the pressure in both reactors tracks the nonlinear model before and after the increase in compressor pressure difference (give RMS numbers)
\par The response of the temperature to the increased compressor pressure difference follows a similar pattern as the pressure, where a change in one term in the governing equations results in a change in the state variable until another term grows large enough to balance out the change in the first term. However, here the dynamics are slower, so the process can be seen in Figures \ref{fig:tempA_case1} and \ref{fig:tempA_case2}. Here, the increased reaction rate after the increase in compressor pressure difference results in an increase in the heat released or absorbed by the reaction, pushing the temperature of the hydrides in both reactors away from the temperature of the circulating fluid in their reactors. As the hydride temperature moves away from the circulating fluid temperature, the heat transfer between the reactor and the circulating fluid increases, as seen in Figure \ref{fig:Case1_lin_perf_heat}. This heat grows until it is approximately equal to the heat transfer from the absorption and desorption reactions, at which point the temperature becomes approximately steady. (give a number to quantify the dynamics here- i.e, time for system to reach some near-equilibrium state). Here again, the linear model is largely successful in tracking the nonlinear model, but does noticeably overestimate the change in temperature in reactor B after the step change, as seen in Figure \ref{fig:tempB_case1}. (add RMS numbers here too) 

\par The change in the weight fraction over time is different from that of the temperature and pressure because the weight fraction changes continually and does not go to any near-equilibrium state. The dynamics of the weight fraction are controlled by the reaction rate in each reactor, which is the derivative of the weight fraction in that reactor. As discussed with the pressure dynamics, the reaction rate in both reactors changes quickly in the seconds after the change in compressor pressure difference until the absorption rate in reactor A, the desorption rate in reactor B, and the mass flow between the reactors are approximately equal. This quick change in the reaction rate, with the very slow change for the rest of the time, results in the weight fraction in each reactor resembling a linear function with a different slope after the step change than before, as seen in Figures \ref{fig:weightA_case1} and \ref{fig:weightB_case1}. The linear model follows the nonlinear model in this, with (error numbers)
 
\par For Case 2, despite hydrogen flow in the system moving in the opposite direction, many of the same trends can be seen as in Case 1. In response to the change in compressor pressure difference, there is a rapid change in pressure, primarily in Reactor A due its reaction rate being less sensitive to pressure, seen in Figures \ref{fig:pressA_case2} and \ref{fig:pressB_case2}. The temperature in both reactors moves away from the circulating fluid temperature, leading to increasing heat rates until these balance out the heat released by the reaction in reactor A and absorbed by the reaction in reactor B. This can be seen in , seen in Figures \ref{fig:tempA_case2}, \ref{fig:tempB_case2}, and \ref{fig:Case2_lin_perf_heat}. Finally the weight fraction, shown in , seen in Figures \ref{fig:weightA_case2} and \ref{fig:weightB_case2}, is approximately linear with respect to time both before and after the increased compressor pressure difference, with the magnitude of the slope increasing after the change due to the change in reaction rates with the change in reactor pressures.
\par However, the linear model does track the nonlinear model as well in this case. (Give numbers).

\subsection{Resetting the Linearization Point}

\par For longer time periods, there is a significant concern about whether the linear model will accurately track the nonlinear model as operating conditions move further away from those at the linearization point. Thus, the linear approximation becomes less accurate. To address this, the linear model can be periodically re-linearized around the current operaing condition.  To illustrate how re-linearization affects the accuracy of the linear model, we consider the evolution of the system for 100 minutes starting with the initial conditions shown in Table~\ref{tab:in_var_relin} using both the nonlinear model and the linear model. In order to sustain the absorption and desorption reactions in the reactors for 100 minutes, the compressor pressure difference is increased by 10 kPa every 10 minutes. We compare three different cases: 1) simulating the linear model from the same initial conditions without any re-linearization, 2) simulating the linear model beginning with the same initial conditions but then relinearizing it every 10 minutes, and 3) repeating case 2 but also resetting the state variables to match the nonlinear model at the time of relinearization. The resulting heat transfer rates for these cases are compared against the nonlinear model simulation in Figure~\ref{fig:Qout_relin_with_no_relin}.

\begin{table}[!htb]
\caption{Initial values for the state and input variables for comparing performance with and without re-linearizing the model and for the case where the controller is used for flow from reactor B to reactor A.} 
\begin{center}
%\small
  \begin{tabular}{l c c l c c}
  \noalign{\vskip -1.5mm}
  \hline
  \noalign{\vskip 1mm}
  $\textbf{\text{Variable}}$ & $\textbf{\text{Value}}$  & $\textbf{\text{Units}}$ & $\textbf{\text{Variable}}$ & $\textbf{\text{Value}}$  & $\textbf{\text{Units}}$\\
  \noalign{\vskip 1mm}
  \hline
  \noalign{\vskip 1mm}
    $T_{i,A}$ & 6.9 & \degree C & $\dot{m}_{A}$  & 0.2 & kg/s \\
    $T_{i,B}$ & 37. & \degree C & $\dot{m}_{B}$  & 0.2 & kg/s \\
    $P_{i,A}$ & 480 & kPa & $\Delta P_{comp}$  & 210 & kPa \\ 
    $P_{i,B}$ & 280 & kPa & $T_{wg,in,A}$ & 1.9 & \degree C\\
    $w_{i,A}$ & 0.004 & kg H / kg M & $T_{wg,in,B}$ & 42. & \degree C \\
    $w_{i,B}$ & 0.0095 & kg H / kg M & & & \\
  \noalign{\vskip 1mm}
  \hline
  \end{tabular}
\end{center}
\label{tab:in_var_relin}
\end{table}
%THERE'S A PROBLEM HERE; NEED TO FIX THE FIGURES
\begin{figure}[!htb]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Relin_case_heatA.jpg}
         \caption{Reactor A: All cases}
         \label{fig:heatA_relin}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Relin_case_heatA_all_relin.jpg}
         \caption{Reactor A: No case without re-linearization}
         \label{fig:heatA_relin_all_relin}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Relin_case_heatB.jpg}
         \caption{Reactor B: All cases}
         \label{fig:heatB_relin}
     \end{subfigure}
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Relin_case_heatB_all_relin.jpg}
         \caption{Reactor B: No case without re-linearization}
         \label{fig:heatB_relin_all_relin}
     \end{subfigure}
     \caption{Heat transfer rates from the hydride beds to the circulating fluid. The performance of the linear models is compared to the nonlinear model (solid black line) for three different cases: one where the model is never re-linearized (dot-dashed pink line), one where it is re-linearized every 10 minutes (dotted blue line), and one where it is re-linearized and reset to match the target every 10 minutes (dashed red line). Throughout this study, the compressor pressure difference is increased by 10 kPa every 10 minutes.}
    \label{fig:Qout_relin_with_no_relin}
\end{figure}

Without re-linearization, the linear model sharply diverges from the nonlinear model until its output eventually bears no resemblance to it, but the periodic re-linearization prevents this from happening. Both re-linearizing and re-linearizing and resetting to match the nonlinear model result in comparable predictions after $\sim$20 minutes. The linear model diverges within the first 10 minutes, but approaches the nonlinear model after the first re-linearization and continues to agree well for the remainder of the simulation. This indicates that the linear model is less accurate when linearized around the initial condition for this case than when linearized around any subsequent point. This is primarily due to the initial reaction rate in reactor B being an order of magnitude larger than the initial rate in reactor A, whereas at all subsequent linearization points are much closer to being balanced. Not re-linearizing the model does not lead to significant divergence if $T_{i,B}$ is reduced to 35 $\degree$C, since this changes the initial reaction rate to be approximately equal to that in reactor A. Re-linearization is therefore less important for some initial conditions than others. The primary advantage of re-linearization is to avoid a case where the linear model diverges sharply from the nonlinear model because it was linearized around an initial point where the rate of change of mass and energy are much larger than they are for most of the operating time. 
